A Hierarchical Descriptor Framework for On-the-Fly Anatomical Location Matching between Longitudinal Studies

We propose a method to match anatomical locations between pairs of medical images in longitudinal comparisons. The matching is made possible by computing a descriptor of the query point in a source image based on a hierarchical sparse sampling of image intensities that encode the location information. Then, a hierarchical search operation finds the corresponding point with the most similar descriptor in the target image. This simple yet powerful strategy reduces the computational time of mapping points to a millisecond scale on a single CPU. Thus, radiologists can compare similar anatomical locations in near real-time without requiring extra architectural costs for precomputing or storing deformation fields from registrations. Our algorithm does not require prior training, resampling, segmentation, or affine transformation steps. We have tested our algorithm on the recently published Deep Lesion Tracking dataset annotations. We observed more accurate matching compared to Deep Lesion Tracker while being 24 times faster than the most precise algorithm reported therein. We also investigated the matching accuracy on CT and MR modalities and compared the proposed algorithm's accuracy against ground truth consolidated from multiple radiologists.

==> ablations.tex <==


\subsection{Ablation Studies}

%In this section, we have conducted experiments with different configurations of the proposed method to investigate the contribution of different parts.  

\subsubsection{Distance Metrics}

\begin{table*}
\centering
	\caption{Median distance errors for distance metrics}
	\setlength{\tabcolsep}{3pt}
	\begin{tabular}{|p{70pt}|p{70pt}|p{70pt}|p{70pt}|p{70pt}|}
		\hline
		Name & Cosine & Euclidean &  Mutual Info & Combined\\
		\hline
		Aneurysm & 3.952 & 4.74 & 4.526  & 4.241  \\
		Lung Nodules     & 1.136 & 1.19 & 1.136 &  1.136 \\
		Kidney Lesions   &  3.454 & 3.536 & 3.078 & 3.078  \\
		ICA                   & 1.611 & 9.417 & 2.374 & 0.922  \\
		Lymph Nodes     & 4.146 & 3.814 & 3.084 & 3.288  \\
		Meningioma       & 1.793 & 2.154 & 1.604 &1.62  \\
		All                    & 2.78   & 3.095 & 2.493 & 1.685  \\
		
		\hline
	\end{tabular}
	\label{table:sim}
\end{table*}


	Many distance measures are usable for our algorithm. In this experiment,  we mainly investigated three of them: cosine, euclidean, and mutual information. In our experiments, we have used a combination of cosine and mutual information measures, so the combined measure is added to the comparison. The median matching distances are given in Table \ref{table:sim}. Overall best performing method is combined distance as expected. Euclidean is not robust in MR studies and underperforms against other distance measures. Mutual info is overall the best individual similarity measure; however, it is the most computational one compared to others. Adding Euclidean similarity to the combined score had a negligible mixed effect on performance, thus excluded in the final combined score. 
	
	%We experimented with different configurations of the proposed method to investigate the contribution of different parts. 

	% In the proposed method both cosine similarity and mutual information is used. We have compared these distance metrics separately in Table \ref{table:sim}. 
	
	%It is visible that two distance metrics are better. More degradation occurs if mutual information is removed from MRI studies. Whereas cosine similarity is more important in CT studies. 

	%Overall distance metrics performs similar on median. However, Euclidean is not robust in MR studies. 

	%Mutual information is slower than the other two. Adding euclidean has a minor effect thus not added in final metric. 

% Comment
\iffalse
Cosine Only:
{'AOR': (0.764, 3.952, 6.326),
 'PULM': (0.911, 1.136, 2.099),
 'KID': (0.709, 3.454, 16.626),
 'ICA': (0.505, 1.611, 24.286),
 'LN': (0.65, 4.146, 9.328),
 'MEN': (0.822, 1.793, 5.687),
 'All': (0.731, 2.78, 10.743)}

Mutual info Only:

{'AOR': (0.708, 4.526, 56.223),
 'PULM': (0.899, 1.136, 14.865),
 'KID': (0.744, 3.078, 34.739),
 'ICA': (0.491, 2.374, 47.786),
 'LN': (0.654, 3.084, 33.909),
 'MEN': (0.768, 1.604, 23.632),
 'All': (0.716, 2.493, 36.195)}

Euclidean:
{'AOR': (0.683, 4.74, 11.596),
 'PULM': (0.905, 1.19, 2.233),
 'KID': (0.716, 3.536, 15.687),
 'ICA': (0.499, 9.417, 23.093),
 'LN': (0.719, 3.814, 7.009),
 'MEN': (0.662, 2.154, 27.036),
 'All': (0.702, 3.095, 14.028)}

{'AOR': (0.792, 4.74, 11.596),
 'PULM': (0.953, 1.19, 2.233),
 'KID': (0.816, 3.536, 15.687),
 'ICA': (0.6, 9.417, 23.093),
 'LN': (0.857, 3.814, 7.009),
 'MEN': (0.712, 2.478, 27.199),
 'All': (0.793, 3.125, 14.05)}


Both:
{'AOR': (0.811, 4.241, 4.599),
 'PULM': (0.951, 1.136, 1.093),
 'KID': (0.817, 3.078, 9.969),
 'ICA': (0.929, 0.922, 4.188),
 'LN': (0.694, 3.288, 7.984),
 'MEN': (0.894, 1.62, 2.984),
 'All': (0.851, 1.685, 5.207)}


{'AOR': (0.906, 4.241, 4.599),
 'PULM': (0.976, 1.136, 1.093),
 'KID': (0.897, 3.078, 9.969),
 'ICA': (0.95, 0.922, 4.188),
 'LN': (0.838, 3.288, 7.984),
 'MEN': (0.938, 1.62, 2.984),
 'All': (0.919, 1.685, 5.207)}


All combined:
{'AOR': (0.807, 3.97, 4.71),
 'PULM': (0.951, 1.136, 1.093),
 'KID': (0.805, 2.845, 10.398),
 'ICA': (0.871, 0.945, 7.385),
 'LN': (0.696, 3.247, 7.893),
 'MEN': (0.894, 1.62, 2.984),
 'All': (0.839, 1.699, 5.804)}



{'AOR': (0.899, 3.853, 4.952),
 'PULM': (0.975, 1.144, 1.104),
 'KID': (0.869, 3.017, 11.115),
 'ICA': (0.819, 0.927, 12.821),
 'LN': (0.827, 3.502, 8.511),
 'MEN': (0.937, 1.729, 3.001),
 'All': (0.89, 2.091, 6.931)}
 
 {'AOR': (0.811, 4.241, 4.599),
 'PULM': (0.951, 1.136, 1.093),
 'KID': (0.817, 3.078, 9.969),
 'ICA': (0.929, 0.922, 4.188),
 'LN': (0.694, 3.288, 7.984),
 'MEN': (0.894, 1.62, 2.984),
 'All': (0.851, 1.685, 5.207)}


\fi

	


\subsubsection{Search Levels}

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{img/levels.png}
	\caption{ROC with different search levels from 1 to 6 }
	\label{fig:levels}
\end{figure}

Another configuration element in our method is the number of levels in the hierarchical search operation. In order to investigate the effect of this selection, we have changed the number of levels from 1 to 6 in this experiment using our mixed modality data.

 Each level comes with a computational cost with a diminishing effect on performance improvement. Increasing the number of levels is beneficial up to level 5, as shown in Figure \ref{fig:levels}. Adding 6th level harms instead of helping. One reason is that at level 6, the field of view reduces to a 12mm radius which is not a very effective descriptor for matching. Computational time increases with an increasing number of layers. Including only the first level took 58ms, whereas including up to the 6th level took 170ms on average in our experiment using the mixed modality dataset. 




\iffalse

[('current_point', 'LevelExperiments.png', 0.061, 73.414, 265.961, 0.18, 0),
 ('FastSearchMapper1', 'LevelExperiments.png', 0.539, 9.926, 13.822, 0.924, 0),
 ('FastSearchMapper2', 'LevelExperiments.png', 0.71, 5.502, 8.464, 0.967, 0),
 ('FastSearchMapper3', 'LevelExperiments.png', 0.782, 3.592, 6.937, 0.967, 0),
 ('FastSearchMapper4', 'LevelExperiments.png', 0.832, 2.263, 5.571, 0.972, 0),
 ('FastSearchMapper5', 'LevelExperiments.png', 0.851, 1.685, 5.207, 0.976, 0),
 ('FastSearchMapper6', 'LevelExperiments.png', 0.834, 2.15, 5.649, 0.976, 0)]

plt.plot(np.arange(1,21), times);plt.xlabel('# Threads');plt.ylabel('Time(s)')

\fi

\iffalse
\subsection{Alternative Models}

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{img/pointmatchingmodels2.png}
	\caption{Operating points of alternative sampling models}
	\label{fig:models}
\end{figure}

    Hierarchy has the advantage of using fewer resources with a bigger field of view. However, it is still interesting to see how alternative sampling approaches perform to compare against our hierarchical model. In this ablation study, we have used models with random sampling locations and sampling points from a regular grid on world coordinates. Random models are parameterized with maximum field of view in millimeters, whereas grid models are parameterized with grid spacing. We used 11x11x11 points in the grids. Additionally, we have added alternative hierarchical grid models with a similar number of dimensions. The results are illustrated in Figure \ref{fig:models} in terms of median error distance and elapsed time.

    The hierarchical models outperform estimation accuracy while having comparable runtime with grid models.   We have used alternative hierarchical models with a different number of grid points in each level from 5 to 11. The difference is less than 0.5mm among them. Uniform grid models are usually faster in estimation, while their best configurations are comparable in estimation accuracy. Our selected model is the best tradeoff between accuracy and speed in alternative models. 
\fi

\subsubsection{Parallelization Performance}



In many cases, multicore parallelization is commonly available in clinical workflow computers despite the lack of access to GPU resources. However, it is still interesting to investigate the runtime behavior of different CPU hardware configurations. Thus, we have changed the number of threads from 1 to 20 in our CT, MR dataset. With 1 thread average computational time for single point matching is 0.74s, whereas, at 20 threads, it becomes 0.16s per volume. However, increasing the number of threads above 12 threads has negligible improvement as in Figure \ref{fig:speed}. 

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{img/Time.png}
	\caption{Computational time of matching with increasing number of threads}
	\label{fig:speed}
\end{figure}	

%Ablations:	Metrics, Features, Parallelization
%Ablation of Search Levels
%Ablation of Metrics 
%- I wonder how the speed-performance would be in 2mm iso subvolumes
%- Parallelism and scaling 


\iffalse
plt.plot(range(1, 21), times, linewidth=2);plt.xticks(range(1,21));plt.grid();plt.show()

[0.7379155226793335,
 0.42090640813818475,
 0.3564868945081087,
 0.3151670157626907,
 0.2770579832990023,
 0.24719829807914265,
 0.23604008145806912,
 0.20730575340054047,
 0.19593908662479637,
 0.1897558002110341,
 0.18361241218603053,
 0.17225880871451862,
 0.16923211423141696,
 0.1697195435022291,
 0.16928675615392025,
 0.16746629357902926,
 0.1686662429881887,
 0.16746328792300835,
 0.162011617732839,
 0.16026299372668515]

\fi


==> removed.tex <==
For example, there is only a single finding per study in three brain MRI studies, as shown in Figure \ref{fig:timepoints}. 


 \begin{figure} 
	\centering
	\includegraphics[scale=0.26]{img/taskexample.png}
	\caption{A longitudinal study of brain MRI with a single finding across time points} 
	% Multiple Time Points 
	\label{fig:timepoints}
\end{figure}	


In this study, we demonstrate a novel and efficient descriptor-search based anatomical point matching method in medical images. We have achieved fast runtime by creating sampling-based descriptors and hierarchical search methods. Unlike machine learning approaches, our method does not require any preprocessing, initialization, or training steps. Also, since it is not optimized for a specific dataset, it provides better generalization to multiple modalities and body parts.


\section{Related Work}

	In a recent publication, Banani et al. \cite{el2021bootstrap} have shown that random CNN features without training provide a strong baseline for point cloud registration. They have further improved the performance using unsupervised SimSiam-based \cite{chen2021exploring} representation learning while bootstrapping from these random CNN-based correspondences. Furthermore, Niv et al. demonstrated that even the generative ability of GANs could be replaced by tailored nearest neighbor search \cite{granot2022drop}. These studies indicate that learning is not always essential in matching problems. 
 

	Traditional deformable registration methods have shown utility in different modalities and anatomical regions. Typically, registration formulation is an optimization of a loss function that combines image similarity and deformation field regularization. These methods tend to be slow during optimization due to a large number of parameters. Only in a recent work, iterative image registration between CT images is reduced to about 5 seconds on the CPU \cite{hansen2021revisiting}.
	
	%Traditional deformable registration methods have shown benefits in different modalities and anatomical regions. Typically, the formulation is an optimization of a loss function, which is a combination of similarity and regularization based on the deformation field. They tend to be slow in optimizing due to the large number of parameters. In only a recent study, iterative image registration between CT images is reduced to about 5 seconds on the CPU.
	
	
	Deep learning approaches have improved the computational time of iterative deformable registration methods by learning deformation estimation functions from given pair of images  \cite{balakrishnan2019voxelmorph,huang2021coarse,guo2019multi,hasenstab2021cnn,mok2020large,czolbe2020deepsim}. These methods carry part of the computational time from runtime to training time. However, the optimized network would be optimal only for the dataset types that are present in training. Thus, domain shift adaptation, transfer learning, and noise robustness are ongoing research areas \cite{varoquaux2022machine,tang2022self}. Notably, SynthMorph eliminated the need for real data for registration by synthesizing artificially generated images \cite{hoffmann2021synthmorph} which extends the generalization beyond the modalities in the training data. Still, the registration accuracy depends on the simulation quality, which requires additional care. Unsupervised deep learning methods addressing \cite{chen2021vitvnet,chen2021transmorph} registration problem have improved registration performance with transformer models by allowing a larger receptive field of views. On the other hand, similar limitations would also be prevalent in these architectures.
	
	%Another related area of study is utilizing regression for coordinate normalization that could be used for registration \cite{meine2019efficient,yan2018unsupervised}. These methods allow coarse alignment of the images on the z-axis by mapping them into a normalized coordinate system. They still need additional steps to have complete matching.  \nocite{li2019mvp}
	
	%If the global context is used, the proposed approach is similar to rigid registration methods. For the local approaches, the computational time trade-off will be prevalent. Additionally, similar domain shift problems exist in various self-supervised machine learning methods.

	Landmarking is another methodology to establish the correspondence between pairs of images. However, due to the non-rigid structure of the human body, landmark estimations would not be very accurate in the regions far from the landmarks. Also, increasing the number of landmarks would add to the computational time. Florin et al. reduced this computational time by introducing a reinforcement learning-based search mechanism in landmark localizations \cite{ghesu2017robust}. On the other hand, collecting the annotations and training these detectors are not easily scalable. 






\section{Discussions and Future Work}

In the comparison between medical imaging studies, clinical navigational tasks focus on a limited number of findings. Thus, our point matching approach could be utilized to navigate to the same anatomical location between studies quickly. Our algorithm is fast enough for real-time use and effectively provides a non-rigid mapping between pairs of images. If mistakes happen in localization, it allows fast correction by clicking on another neighbor point in a second trial. Thus, we expect point matching to help the radiologists to save time from scrolling unnecessarily in comparison studies without requiring precomputed registration fields.

%In most cases number of findings is only 1 and the size of findings would be larger than reported mean distances.  

%. According to our results, significant portion of these tasks would be covered.

Compared to the prior art, our method does not require a training step since the sampling model is predefined. However, it is possible to extend this approach to have optimization on the sampling model for a given dataset. Optimized sampling locations would allow using a similar search mechanism with a new descriptor definition. On the other hand, optimization will limit the generic purpose descriptor generation model. Additionally, each level of search requires a specific optimization of the model since data distribution changes. Similarly, representation learning algorithms on existing sampling-based descriptors could be applied. However, any neural network on the descriptor has the disadvantage of additional computational cost. 

Our algorithm relies on medical images being consistent in spatial dimensions between different time points. Significant changes in anatomy or pathology in the images will adversely affect the matching performance. Additionally, sampling locations are rotation sensitive. Thus, the correct orientation of image loading needs to be ensured. These are the known limitations of the proposed algorithm, which need to be considered in different applications. 

The runtime speed of the proposed solution could be improved further by eliminating unnecessary grid search points in the target image, for example, points mostly in the air. Additionally, the feature value in the search point in the target image could be informative for neighborhood regions. This additional information could be utilized to improve computational time further. For example, if a candidate location is found with a very strong confidence score, the rest of the search could be skipped to advance to the next level.

In our work, we have compared CT vs. CT and MR vs. MR studies. It would be an interesting future direction to compare CT vs. MR pair datasets to assess performance in a heterogeneous setting. 
